Explainable Intrusion Detection Systems (X-IDS): A Survey of Current Methods, Challenges, and Opportunities

The application of Artificial Intelligence (AI) and Machine Learning (ML) to cybersecurity challenges has gained traction in industry and academia, partially as a result of widespread malware attacks on critical systems such as cloud infrastructures and government institutions. Intrusion Detection Systems (IDS), using some forms of AI, have received widespread adoption due to their ability to handle vast amounts of data with a high prediction accuracy. These systems are hosted in the organizational Cyber Security Operation Center (CSoC) as a defense tool to monitor and detect malicious network flow that would otherwise impact the Confidentiality, Integrity, and Availability (CIA). CSoC analysts rely on these systems to make decisions about the detected threats. However, IDSs designed using Deep Learning (DL) techniques are often treated as black box models and do not provide a justification for their predictions. This creates a barrier for CSoC analysts, as they are unable to improve their decisions based on the model's predictions. One solution to this problem is to design explainable IDS (X-IDS). This survey reviews the state-of-the-art in explainable AI (XAI) for IDS, its current challenges, and discusses how these challenges span to the design of an X-IDS. In particular, we discuss black box and white box approaches comprehensively. We also present the tradeoff between these approaches in terms of their performance and ability to produce explanations. Furthermore, we propose a generic architecture that considers human-in-the-loop which can be used as a guideline when designing an X-IDS. Research recommendations are given from three critical viewpoints: the need to define explainability for IDS, the need to create explanations tailored to various stakeholders, and the need to design metrics to evaluate explanations.

==> othersampletable.tex <==


\begin{table*}
\centering
{
    \rowcolors{1}{lightgray!20!}{}
    \begin{tabularx}{\textwidth}{X|X|X|X}
    \hline
    \textbf{Category} & 
    \textbf{Focus/Objective} & 
    \textbf{Contributions} & 
    \textbf{Limitations} &
    \hline
    %==========================================%
    
    \hline
\multicolumn{4}{l}{\textit{\textbf{Narrative Extraction}}} \\ 
\hline
    \begin{minipage}[t]{\linewidth}\textbf{Event \\ Detection}\\ \cite{spiliopoulou2017event, das2014frame, rehm2017event, chen2015event} \end{minipage} &
    Identification, tracking, and characterization of event entity types in unstructured and semi-unstructured text data. & Describes approaches to categorize events into types, sub-types through methods such as hierarchical clustering, semantic frame parsing, and large language modeling. &
   \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Lacks statistical abilities to detect events defined implicitly in text.
   \item Performance of methods rely on quality of designed input features, and unable to generalize well. 
   \end{itemize}  
    \vspace{1mm}
    \end{minipage}
     &
    \hline 
    %==========================================%
    \begin{minipage}[t]{\linewidth}\textbf{Relationship Extraction} \\ \cite{oza2021entities,sarawagi2008information,bodrova2014relationship} \end{minipage} &
    Extraction of semantic relationships that exist between named entities. & Methods to link narrative events together based on contextual relationships between entities. &
    Tasks tested on small scale typically limited to domain-specific applications.
     \vspace{1mm}
    &
    
    \hline
    %==========================================%
    \begin{minipage}[t]{\linewidth}\textbf{Narrative Representation Language}\\ \cite{hussain2021stories,yan2019using,gervas2013stories} \end{minipage} &
    Representation of primary components of a narrative through extensible, machine-readable narrative representation structures. &
    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Creation of functional story schemas that capture latent, structural features in unstructured text.
   \item Visualization techniques to display fragmented narrative components in a user interface.
   \item Development of domain-specific narrative schemas.
   \end{itemize}  
   \end{minipage}
    &
   \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Subject bias when forming grammar rules.
   \item Non-generalizable representations.
   \item Schema clustering algorithms easily lose ordering/temporal information.
   \end{itemize}  
   \end{minipage}
     &
    \hline
    \multicolumn{4}{l}{\textit{\textbf{Story Evolution}}} \\
    \hline
    %==========================================%
   \begin{minipage}[t]{\linewidth}\textbf{Shift Detection}\\
\cite{hussain2018analyzing,marcoux2021narrative}
\end{minipage} &
    Identifies transitions between plot elements.
    
    &
    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Methods to study shifts in narratives across disparate online sources.
   \item Topic Modeling to assess shifts in narrative sentiments
   \item Extraction of chronological themes across social media narratives.

   \end{itemize}  
   \end{minipage}
    &
    
    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Non-generalizable models.
   \item Scalability issues.
   \item Temporal expression limited to dates and \\timestamps.

   \end{itemize}  
   \end{minipage}
    &
    \hline
    %==========================================%
    \begin{minipage}[t]{\linewidth}\textbf{Storyline Construction}\\
\cite{shahaf2010connecting,fung2007time,nallapati2004event,mei2005discovering,croft2017integrating,zhu2012finding}\end{minipage} &
    Create methods for sequencing causal events and temporal narrative shifts.
    
    &
   \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Event decomposition methods to represent storylines as evolving sets of subevent interactions.
   \item Formation of story chains.
   \item Ordering of online sources based on hierarchal structures.


   \end{itemize}  
   \end{minipage}
    &
    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Targeted inputs with known start and end to \\storyline.
   \item Does not study the potentials of reordering of events based on new information.
   \item Limited analysis on unrealized events in annotations and representations.
   \end{itemize}  
   \end{minipage}
    &
    \hline
    %==========================================%
    \begin{minipage}[t]{\linewidth}\textbf{Timeline Generation and Summarization}\\
\cite{chieu2004query,lin2008storyline,yan2011evolutionary,pasquali2019interactive,mccreadie2018explicit}\end{minipage} & 
     Extracting events and placing them on a chronological timeline, based on a user queries from a collection of documents.
    & 
    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Methods to structurally organize sequential events in both graphical and timeline formats.
   \item Producing evolutionary summaries (evolution trajectory) of events.

   
   \end{itemize}  
   \end{minipage}
    & \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Does not take into consideration aspects such as bias and hyperpartisan augmention.
   \item ost systems developed \\worked independently of an integrated search engine.

   
   \end{itemize}  
   \end{minipage} 
    &
    \hline
    %==========================================%
   \begin{minipage}[t]{\linewidth}\textbf{Causal Relation Extraction and Arrangement}\\
\cite{mori2021nectar,hu2017inference}
\end{minipage} & Identifying cause/effect relationships between narrative events. & \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Methods that predict position of missing narrative components, given incomplete story inputs.
   \item Augmentation of current baseline datasets to learn additional fine-grained causal relations.

   
   \end{itemize}  
   \end{minipage} &    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Experimentation on short stories, minimizing contextual feature space.
   \item Domain-specific experiments not generalizable.

   \end{itemize}  
   \end{minipage} &
    \hline
    \rowcolor{white}
    \multicolumn{4}{l}{\textit{\textbf{Narrative Generation}}} \\
    \hline
    %==========================================%
    \rowcolor{lightgray!20!}
    \begin{minipage}[t]{\linewidth}\textbf{Structural Methods}\\
\cite{fan2018hierarchical,martin2018event}\end{minipage} &
    Preprocessing narrative text into structures such as sequences or hierarchical graphs and later decomposed into task-oriented text generation. &
    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Generation of linguistically coherent text given an incomplete narrative structure as input.
   \item Using sequential learning to preprocess textual story data into event sequences.
   \item Methods to reduce sparsity of events to maintain semantic meaning of textual story data.

   
   \end{itemize}  
   \end{minipage} &
    \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Introduces sub-problem of potentially unreadable output.
   \item Random sampling can occasionally miss important tokens.
   \item Sequence modeling introduces content repetition as output is generated.

   
   \end{itemize}  
   \end{minipage} &
    \hline
    %==========================================%
     \rowcolor{white}
   \begin{minipage}[t]{\linewidth}\textbf{Goal-oriented Methods}\\
\cite{li2021using,mao2019improving}
\end{minipage} & Improving generated text in logical, stylistic, event-driven, and context-driven scopes. &   \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Editing beam search mechanisms to generate likely next sentence based on logical context.
   \item Increased logical coherency of generated text.
   

   
   \end{itemize}  
   \end{minipage} &  \begin{minipage}[t]{\linewidth}
   \begin{itemize}[nosep, wide=0pt, leftmargin=*, after=\strut]
   \item Lack of characterization of narrative actors in generation pipelines.
   \item Frame Parsers fail at processing complex sequences.
   \item Reliance on short-term common sense grounding poses limitations on achieving story-level coherence.
   

   
   \end{itemize}  
   \end{minipage} &
    %\hline
    \end{tabularx}
}
\caption{Computational Understanding of Narratives: Current Research and Open Challenges}
\label{table:existing_research}
\end{table*}


==> tableblackbox.tex <==
\begin{table*}
\centering
{
   % \rowcolors{1}{lightgray!20!}{}
   %\rowcolors{1}{cyan!20!}{}
   {\renewcommand{\arraystretch}{1.30}%
    \begin{tabularx}{\textwidth}{X|X|X|X}
    \hline
    \rowcolor{lightgray!20!}
    \textbf{Paper Title} &
    \textbf{Focus/Objective} &
    \textbf{Contribution} &
    \textbf{Limitation} \\
    \hline
    %==========================================%
    \rowcolor{cyan!20!}
    \multicolumn{4}{c}{Feature based IDS} \tabularnewline
    \hline
     %==========================================%
    An Explainable Machine Learning Framework for Intrusion Detection Systems \cite{wang2020explainable} &
    Locally and globally explainable NN using SHAP for IDS. &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
      \item Framework that creates both local and global explanations.
      \item First use of SHAP in the field of IDS.
      \item Comparison between one-vs-all classifier and multi-class classifier.
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item More intrusion detection datasets should be tested.
        \item SHAP cannot work in real-time.
        \item SHAP needs to be tested on more robust attacks.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    %==========================================%

    Domain Knowledge Aided Explainable Artificial Intelligence for Intrusion Detection and Response \cite{islam2019domain} &

    Use CIA principles on data to improve both generalizability and explainability of a model &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Method for the collection and use of Domain Knowledge in IDS
      \item Use CIA principles to aid in explainability
      \item Domain Knowledge increase generalizability
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Domain Knowledge is applied to a specific dataset. New mappings may be needed on new datasets.
        \item More datasets need to be tested.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    %==========================================%

     An Explainable Machine Learning-based Network Intrusion Detection System for Enabling Generalisability in Securing IoT Networks\cite{Sarhan2021AnEM} &

    Explore explainability in IDS by comparing two different IDS feat.  &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Evaluate twe different Network Intrusion Detection datasets: NetFLow and CICFlowMeter.
      \item Creation of two new datasets in the CICFlowMeter format.
      \item An explainable analysis is performed using SHAP.
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Explanations are only done using SHAP.
        \item No analysis on the performance of the explainer.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    %==========================================%

    Explaining Anomalies Detected by Autoencoders Using SHAP\cite{Antwarg2019ExplainingAD} &

    Use SHAP to create custom explanations for anomalies found with an autoencoder. &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Method for explaining anomalies found by an autoencoder.
      \item Preliminary experiment with real word data and domain experts.
      \item Suggest methods for evaluating explanations.
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Custom explanation lacks any form of visualization to aid the user.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    %==========================================%
    \rowcolor{cyan!20!}
    \multicolumn{4}{c}{Perturbation based IDS} \tabularnewline
    \hline

    A New Explainable Deep Learning Framework for Cyber Threat Discovery in Industrial IoT Networks \cite{khan2021new} &

    Explainable Intrusion Detection in the field of IoT &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Conv-LSTM-based autoencoder for time-series attacks
      \item Detects zero-day attacks
      \item Sliding window technique that increases accuracy of CNN and LSTM model XAI concepts to improve trust
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Tested only on a single dataset
        \item Considers only univariate time-series data
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    %==========================================%

    An Adversarial Approach for Explainable AI in Intrusion Detection Systems \cite{marino2018adversarial} &

    Explain models and predictions through an adversarial approach  &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Methodology explaining incorrectly classified samples to help improve flaws in the model
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Only tested on DoS attacks from NSL-KDD
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    %==========================================%

    Feature-Oriented Design of Visual Analytics System for Interpretable Deep Learning Based Intrusion Detection \cite{wu2020feature} &

    A suite of visual tools used to improve explainability of CNNs  &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Analysis of Features and Requirements to improve visual analysis of XAI
      \item IDSBoard, a GUI for understanding Deep Learning Intrusion Detection
      \item Demonstrate the effectiveness of visual analytics
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Only tested on a single dataset
        \item Scalability of visual analytics system
        \item Visual analytics system only designed for CNN
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline

    %==========================================%

    Explanation framework for Intrusion Detection \cite{burkart2021explanation} &

    Explaining IDS explanations using a Counterfactual technique.  &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Explaining classifications based on feature importance.
      \item Advice on how to change a classification to its desired result.
      \item Outline the decision process so that the user can simulate it themselves.
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Analysis of the counterfactual technique was only run on one type of ML algorithm.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
    \\
    \hline
    %==========================================%
    \rowcolor{cyan!20!}
    \multicolumn{4}{c}{Decomposition/Gradient based IDS} \tabularnewline
    \hline

    Toward Explainable Deep Neural Network Based Anomaly Detection. \cite{amarasinghe2018toward} &

    Initial steps into XAI for DNN Intrusion Detection &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item Framework for creating an explainable Deep Network XAI concepts to improve trust
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Experiments are run using only DOS attacks from the NSL-KDD dataset
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    
\end{tabularx}
}

\caption{An overview of the existing literature on black-box approaches to intrusion detection systems, with a focus on their scope, contribution, and limitations. (Continued)} 
\label{table:blackbox_table}

\end{table*}

\addtocounter{table}{-1}

\begin{table*}
\centering
{
    
    {\renewcommand{\arraystretch}{1.30}%
    \begin{tabularx}{\textwidth}{X|X|X|X}
    \hline
      %==========================================%

    Towards explaining anomalies: A deep Taylor decomposition of one-class models. \cite{Kauffmann2020TowardsEA} &

    Explaining anomalies found by a SVM using Deep Taylor Decomposition.  &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

      \item A method for `neuralizing' a one-class SVM to be explained by Deep Taylor Decomposition.
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Experiments solely run using one-class SVM. No comparison to `real' neural networks.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
    %==========================================%
  
   %==========================================%
   \rowcolor{cyan!20!}
   \multicolumn{4}{c}{Hybrid IDS} \tabularnewline
   \hline
    Achieving explainability of intrusion detection system by hybrid oracle-explainer approach  \cite{szczepanski2020achieving} &
    Building a hybrid IDS based around `XAI Desiderata' that does not decrease performance or add vulnerability.  &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
      \item An explainer module modeled after the `XAI Desiderata.'
      \item A Hybrid-Oracle explainer Intrusion Detection System.
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]

        \item Two models need to be effectively trained.
        \item Would benefit from being tested on multiple datasets.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline
  
    %==========================================%
      
    Explainable deep few-shot anomaly detection with deviation networks \cite{pang2021explainable} &
    An anomaly detection system able of detecting anomalies learned from few anomalous training samples.  &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
      \item Prior-driven anomaly detection framework.
      \item DevNet, an anomaly detection framework based on Gausian prior, Z-Score-based deviation loss, and multiple instance learning.
      \item A theoretical and empirical analysis of Few-shot anomaly detection.
    \end{itemize}
    \vspace{1mm}
    \end{minipage} &
    \begin{minipage}[t]{\linewidth}
    \begin{itemize}[leftmargin=*]
        \item Experiments only run using image based datasets with relatively small sample sizes.
    \end{itemize}
    \vspace{1mm}
    \end{minipage}
     \\
    \hline 
    \end{tabularx}
}
\caption{An overview of the existing literature on black-box approaches to intrusion detection systems, with a focus on their scope, contribution, and limitations. (Continued)}}
\end{table*}


==> whitebox.tex <==

\subsection{White Box X-IDS Models}
%\hl{for each subcategory add a note on explainability}

%Machine learning models that provide results associated with their models that are easily interpreted, explained, and understood by domain knowledge experts are referred to as an understandable model, XAI, and white box. Typically, these models offer a good balance of accuracy and explainability \cite{rudin2019stop}.

Models that can provide an explanation to expert users without utilizing additional models are referred to as \textit{interpretable} or \textit{white box models} \cite{loyola2019black}. A white box model’s internal logic and programming steps are completely transparent, resulting in an interpretable decision process \cite{pintelas2020grey}. However, when the model is to be explained to non-expert users, it may demand post-hoc explainability, such as visualizations \cite{arrieta2020explainable}. This interpretability, on the other hand, usually comes at a price in terms of performance \cite{islam2021explainable}.

%Most of the described white box studies concentrate more on the accuracy of the various classification algorithms for improved IDS performance. They were \textit{not designed} from an interpretability standpoint which is why they do not provide insights into their behavior and reasoning for the predicted outcome. However, to understand the prediction output of these models we can use feature importance plots such as SHAP summary plots. By constructing such a plot, we can easily understand global feature importance from the entire training dataset. For instance, in the NSL-KDD dataset “class” feature is used to differentiate between benign and malicious traffic, so if malicious traffic is detected in the given set of input data, the analysis of the features that are helping to detect malicious traffic would be highly beneficial explaining why that traffic is malicious.

A myriad of white box approaches are available for intrusion detection. Our survey will focus on the approaches most commonly used in the literature, as per our overview presented in Section \ref{overview}  and the taxonomy showcased in Figure \ref{tax_fig}. Table \ref{table:existing_research_white_box} summarizes state-of-the-art research, challenges, and
contributions with respect to white box approaches for intrusion detection systems. 
 %such as Regression, Decision Tree, Rule-based, Statistical and Probabilistic Models, and Clustering. 

\input{whitebox_tables}

\subsubsection{Regression} Linear Regression (LR) is a supervised ML technique that establishes a relationship between a dependent variable and independent variables by computing a \textit{best fit} line. The linearity of the learned relationship puts LR under the umbrella of interpretable models. Intrinsically interpretable models such as LR and Logistic Regression (LoR), meet the characteristics of transparent models (algorithmic transparency, decomposability, and simulatability) \cite{lipton2018mythos}. In LR, when the number of features is small, the weight or coefficient of the equation can be used for explaining predictions. %However, to maintain the notion of interpretability, the variables employed in LR and LoR models must be understood by their users \cite{arrieta2020explainable}. 
The learned relationships are linear and can be expressed for a single instance \textit{i} as given in Equation \ref{eq:regression_equation}. %Figure \ref{fig:regression}, illustrates a straightforward linear regression equation for a single variable. We can use the line to calculate y, our target, for any value of x.

%Linear Regression (LR) is a supervised machine learning technique that is generally used for solving regression problems. These models are used to predict continuous dependent variables using independent variables. The objective of the LR model is to find the best fitting line that accurately predicts the output of the continuous dependent variable. The algorithm establishes the linear relationship between the dependent variable and the independent variable by finding the best fit line. The linearity of the learned relationship puts LR under the umbrella of interpretable models. The most convenient way to achieve interpretable results is to stick to intrinsically interpretable models such as LR and Logistic Regression (LoR) as both meets the characteristics of transparent models (algorithmic transparency, decomposability, and simulatability \cite{lipton2018mythos}). The weighted sum of input features determines the predicted target in LR. When the number of features is small, the weight or coefficient of the linear equation can be used as a medium for explaining prediction. The learned relationships are linear and can be expressed for a single instance \emph{i} as given in Equation \ref{eq:regression_equation}. The graph \ref{fig:regression} illustrates a straightforward linear regression equation for a single variable. We can use the line to calculate y, our target, for any value of x. The features of linear regression have an interpretable linear relationship. %When there are multiple correlated features, however, the distinct feature influence is indeterminable because the individual influences on prediction are no longer additive to the overall prediction.The variables used in LR and LoR models must be understandable by their users and the size of such models should be limited to maintain the notion of interpretability \cite{arrieta2020explainable}. %

\begin{equation}\label{eq:regression_equation}
\hat{y}=\beta_{0}+\beta_{1} X_{1}+\cdots+\beta_{n} X_{n}+\epsilon
\end{equation}
where, 
\begin{quote}
$\hat{y}$ is the output or target (dependent) variable. X is the input (independent) variable. $\beta_{0}$, $\beta_{1}$ are coefficients, and $\epsilon$ is  error term. 
\end{quote}

\begin{comment}

\begin{figure}[h!]
    \centerline{\includegraphics[scale =0.55]{figures/regression.pdf}}
    \caption{Overview of XAI for Regression-based model. The variable x represents a point of interest for which we wish to provide an explanation for the prediction \textit{y = f(x)}.}
    \label{fig:regression}
\end{figure}
%\hl{labels are all messed up}

\end{comment}


%\indent Authors of \cite{subba2015intrusion} deployed anomaly-based intrusion detection systems using two different statistical methods such as Linear Discriminant Analysis (LDA) and LoR. The proposed model was evaluated using the benchmark NSL-KDD dataset. In this work, they compared the performance of their model with other intrusion detection models based on Naïve Bayes (NB), C4.5, and Support Vector Machine (SVM). Experimental results indicated that the proposed model both LDA and LoR performed well with binary class and multi-class classification problems. The performance metrics used in this research are accuracy and detection rate. For multi-class NSK-KDD (with class labels (normal, DoS, R2L, Probe)) dataset the proposed LoR method achieved an average accuracy of 95.13\% and detection rate of 98.74\% higher than NB based models with average accuracy and detection rate of 91.25\% and 87.97\% respectively. On the other hand, the proposed LoR method on binary class with 23 features on NSL-KDD dataset outperformed NB, C4.5, and LDA models with an accuracy of 98.27\% and detection rate of 91.59\%. However, it underperformed when compared to SVM methods which have accuracy and detection rate of 99.63\% and 99.16\% respectively. The computation overhead with LoR and LDA methods is significantly less as opposed to SVM methods. This makes the proposed model efficient in real-time network monitoring and intrusion detection analysis. 

%In the work \cite{wang2014new}, the authors proposed a network anomaly detection system based on an ordinary LR method with two novel metrics Inter-group Traffic Entropy (ITGE) and Inter-group Flow Entropy (IGFE). Even though the performance of the LR model was superior to well-known wavelet-based detection methods, the researchers indicated the performance LR model is susceptible to outliers. To mitigate the impact of outliers, they then proposed a robust regression method instead of the ordinary LR method for anomaly detection \cite{wang2017robust}. The dataset used in this experiment is CERNET (China Education and Research Network). The proposed method is based on heteroscedasticity assumption and Huber loss function as opposed to homoscedasticity assumption and sum of squared errors as loss function in ordinary regression methods. The results of the experiment indicated that the robust regression-based detector model is less susceptible to outliers than the conventional regression-based detector.

Various regression-based  IDS models exist in the literature. Authors in \cite{subba2015intrusion} deployed anomaly-based intrusion detection systems using two different statistical methods: Linear Discriminant Analysis (LDA) and LoR. %The proposed model was evaluated using the benchmark NSL-KDD dataset. In this work, they compared the performance of their model with other IDS models based on Naïve Bayes (NB), C4.5, and Support Vector Machine (SVM). For multi-class NSK-KDD (with class labels (normal, DoS, R2L, Probe)) dataset the proposed LoR method achieved an average accuracy of 95.13\% and detection rate of 98.74\% higher than NB based models with average accuracy and detection rate of 91.25\% and 87.97\% respectively. %On the other hand, on binary class with 23 features, the model outperformed NB, C4.5, and LDA models with an accuracy of 98.27\% and detection rate of 91.59\%. 
While LR models are desirable for intrusion detection purposes, their performance is susceptible to outliers \cite{wang2014new}. To mitigate the impact of outliers, the authors in \cite{wang2017robust} proposed a robust regression method for anomaly detection. The proposed method uses heteroscedasticity and a huber loss function instead of homoscedasticity and sum of squared errors. %The results of the experiment indicated that the robust regression-based detector model is less susceptible to outliers than the conventional regression-based detector.


While the existing approaches render promising outcomes, none of them were designed with \textit{explainability} in mind. To overcome the issue of \textit{explainability} in the area of \textit{hardware performance counter} (HPC) – based intrusion detection, the authors \cite{kuruvila2022explainable} propose an explainable HPC-based Double Regression (HPCDR) ML framework. The study examines two distinct types of attacks: microarchitectural and malware. For the first type of attack, tests are conducted on five distinct datasets: Rowhammer, Flush+Flush, Spectre, Meltdown, and ZombieLoad. For the second attack, two distinct datasets are considered: Bashlite and PNScan. To minimize computational overhead, the proposed study employs Ridge Regression (RR) rather than Shapely values to generate interpretable results. First, the three ML models (RF, DT, and NN) are chosen to evaluate the classification accuracy. Second, the output from these models is perturbed and passed to the first RR model where HPCs are employed as features and weight coefficients are received. These furnished coefficients are run on the second RR model, which identifies the most malicious sample. The authors argue that by utilizing double regression techniques, their proposed method provides transparency, which enables users to locate malicious instructions within the program. %Using double regression techniques, the authors argue it is possible to trace through the source code of the malicious testing data and monitor what specific instructions are being executed, \hl{which ultimately helps in the analysis of the interpretability of the results.}


\subsubsection{Decision Tree and Rule Based} 
A Decision Tree (DT) is a tree structure with decision support system elements based on graph theory.  In contrast to LR and LoR methods, it works even when the relationship between input and output is nonlinear. There are two approaches for constructing decision trees: top-down and bottom-up. The top-down approach, which is based on the divide and conquer strategy, is the most frequently used in the literature \cite{quinlan2014c4}. The decision model built with a top-down approach begins with the root node and splits the root nodes into two disjoint subsets: left child and right child. This process is repeated recursively over child nodes until a stop condition is met \cite{maimon2014data}. In their simplest form, DT possesses three properties that make them interpretable \cite{lipton2018mythos}: simulatability, decomposability, and algorithmic transparency \cite{arrieta2020explainable}. Figure \ref{fig: decision_tree} illustrates a simple DT that detects an attack on a remotely accessible computer system.

A simple rule is typically represented as a logical implication of IF-THEN statements by combining relational statements to form their knowledge \cite{loyola2020explainable}. These rules can be extracted from DT. Rule-based models are considered transparent because they generate rules to explain their predictions. Figure \ref{fig: rule_based} depicts a simple snort rule.


%A Decision Tree (DT) is a tree structure with decision support system elements based on graph theory. The decision model is built top-down in the form of a tree structure, beginning with the (top) root node, and progressing to decision nodes and leaf nodes. The root nodes in DT are significant predictors, whereas the leaf nodes provide a final classification. Decision rules in DT such as simple (IF-THEN-ELSE) conditions are based on splitting criteria. These properties make DT decomposable or algorithmically transparent \cite{arrieta2020explainable}. Figure \ref{fig: decision_tree} depicts a simple DT that detects an attack on a remotely accessible computer system. 

%A Decision Tree (DT) is a tree structure with decision support system elements based on graph theory. DT-based models divide the data multiple times at each node based on a cutoff threshold until it reaches a leaf node. In contrast to LR and LoR methods, it works even when the relationship between input and output is nonlinear, and the features interact with one another (co-relating features). The decision model is built top-down in the form of a tree structure, beginning with the (top) root node, and progressing to decision nodes and leaf nodes. The traversal from the root node to the leaf node depicts how the decision is made in DT. DT are hierarchical structures for decision making, root nodes are significant predictors, whereas the leaf nodes provide a final classification. In their simplest form, DTs are models that can be simulated. Their properties, on the other hand, make them decomposable or algorithmically transparent \cite{arrieta2020explainable}. In essence, DT is a naturally interpretable shallow rule-based model. Decision rules in DT such as simple (IF-THEN-ELSE) conditions are based on splitting criteria. These rules make the model interpretable. Figure \ref{fig: decision_tree} depicts a simple DT that detects an attack on a remotely accessible computer system. The leaf nodes of the tree return the classification result in (attack? YES/NO).





% They chose the DT (Iterative Dichotomiser 3 (ID3) algorithm) technique to ensure interpretability since it uses a human-based decision-making strategy, concluding that the algorithm could rank the relevance of features, providing explainable rules, and reaching an accuracy comparable to state-of-the-art algorithms.

Mahbooba et al. \cite{mahbooba2021explainable} approach the task of developing an interpretable model to identify malicious nodes for IDS using a DT on the KDD dataset. They chose the Iterative Dichotomiser 3 (ID3) algorithm to ensure interpretability because it mimics a human-based decision strategy. The authors demonstrate that the algorithm can rank the relevance of features, provide explainable rules, and reach a level of accuracy comparable to state-of-the-art. Another explainable decision tree model is proposed in \cite{loyola2020explainable} and \cite{frost2020exkmc}, with the latter being an extension of work in \cite{dasgupta2020explainable}.

  \begin{figure}[h!]
    \centerline{\includegraphics[scale =.55]{figures/Dt.pdf}}
    \caption{Simple decision tree for the detection of a user-to-root (U2R) attack on a computer system, attack classified as Yes or No  \cite{staudemeyer2012importance}.}
    \label{fig: decision_tree}
\end{figure}

Sinclair et al. \cite{sinclair1999application} extract rules using a DT and a Genetic Algorithm (GA) for improving the performance of the IDS model. The authors in \cite{ojugo2012genetic} and \cite{chadha2015hybrid} focus on optimizing the IDS model by extracting rules using a GA. To add transparency to the decision process, Dias et al. \cite{dias2021hybrid} proposed an interpretable and explainable hybrid intrusion detection system. The proposed system integrates expert-written rules and dynamic knowledge generated by a DT algorithm. The authors suggest that the model can achieve explainability through the justifications of each diagnosis. Justification of certain predictions is provided in a tree-like format in the form of a suggested rule that provides a more intuitive and straightforward understanding of the diagnosis.

%\hl{The authors suggest that the model can achieve explainability and interpretability through the justifications of each diagnosis. The justification for a certain prediction is provided in the form of a suggested rule.}
%An explainable k-Means and k-Medians clustering is proposed in \cite{dasgupta2020explainable}. An extension of this model, ExKMC was proposed with the aid of the explainable decision tree method in \cite{frost2020exkmc}.  According to the authors, this explanation approach is introduced by generating the smallest binary tree possible (threshold tree) with k leaves. The input data is iteratively divided into k clusters by each node in the tree. They ensure that each such path accesses at most k-1 features by limiting it to k leaves. The explanations were created with the help of k-1 features. An explainable decision tree model (eUD3.5) was proposed by authors in \cite{loyola2020explainable}. In this experiment, the researchers evaluated feature splitting in the tree using compactness and separation of data clusters.

%Mahbooba et al. \cite{mahbooba2021explainable} approached the task of developing an interpretable model to identify malicious nodes for IDS using DT on the KDD dataset. The author uses the Iterative Dichotomiser 3 (ID3) algorithm as their DT. Their dataset consists of 42 attributes out of which 41 are classified further into four different classes such as Basic Features (BF), Content Feature (CF), Traffic Feature (TF), and Host Feature (HF). They use DT’s built-in mechanism to report variable importance. According to the authors feature “count” or V23 (a form of an attack lasting more than 2 seconds), ranked highest from the TF category. Similarly, the second-highest ranked feature is “service” or V3 – from the BF category.  After ranking the features and constructing the tree the authors extracted the rules. They use IF-THEN rules with logical conditions to distinguish whether a class is normal or malicious. The experimental result indicated that the DT algorithm has marginal improvements with other state-of-the-art methods including LR and SVM in terms of performance matrices such as precision, recall, and f-1 score. 

%\hl{merge RL DT-- coming up Subash}\subsubsection{Rule based}

%A model that generates rules to characterize data from which it is intended to learn is referred to as rule-based learning \cite{arrieta2020explainable}. A simple rule is typically represented as a logical implication of IF-THEN statements by combining relational statements \cite{loyola2020explainable} or more complex combinations of simple rules to form their knowledge \cite{arrieta2020explainable}. These models are transparent and interpretable because they usually generate rules to explain their predictions. \textit{Snort} is the world's most widely used open-source rule-based intrusion prevention system (IPS) \cite{roesch1999snort}. It employs a set of rules that help define malicious network activity. These rules are then used to identify packets that match those rules and generate alerts for users \cite{roesch1999snort}, \cite{caswell2007snort}. An example of a simple snort rule is depicted in Figure \ref{fig: rule_based}. 
\textit{Snort} is the world's most widely used open-source rule-based intrusion prevention system (IPS) \cite{roesch1999snort}. It employs a set of rules that help define malicious network activity. These rules are then used to identify packets and generate alerts for users \cite{roesch1999snort}, \cite{caswell2007snort}.
  \begin{figure}[h!]
    \centerline{\includegraphics[scale=0.55]{figures/rule_based.pdf}}
       \caption{A simple rule that detects attempts to access the PHF service via a local web server. Any time such a packet is detected on the network, an alert is sent and the entire packet is logged using the run-time logging mechanism  \cite{roesch1999snort}.}
    \label{fig: rule_based}
\end{figure}

%A hybrid genetic fuzzy rule-based inference methodology that aims to detect network-based misuse detection is proposed in \cite{chadha2015hybrid}. According to the authors, fuzzy logic creates precise and adaptable patterns, while a genetic algorithm based on evolutionary computation aids in achieving an optimal solution. Combining the two schemes improves the robustness of detection systems. The authors used the KDD99 dataset for their experiment. Experimental results suggested that the intended approach outperforms all the existing genetic fuzzy approaches (Michigan, Pittsburgh, and Iterative rule learning) with the recall of 94.6\% as compared to Michigan and Iterative Rule Learning with the recall of 68.2\% and 73.9\% respectively.

%In the other work, Ghosh et al. \cite{ghosh2017network} proposed a network anomaly detection using the fuzzy rule-based classifier (RIPPER). An error correction-based learning procedure is used in the proposed method. The authors use 10\% of the NSL-KDD dataset for experimentation purposes. They applied a 10-fold cross-validation method to validate their model. Results indicated the Fuzzy classifier outperforms SVM and KNN with accuracy, true positive rate, false-positive rate, precision, and f-measure of 99.4\%, 99.4\%, 3.0\%, 99.4\%,99.4\% respectively. The high accuracy in the proposed model, however, could be because of overfitting which the author fails to explain in the paper. 

%Sinclair et al. in \cite{sinclair1999application} extracted rules using DT and Genetic Algorithm (GA) for improving the performance of the IDS model, while the authors in \cite{ojugo2012genetic} and \cite{chadha2015hybrid}, focus on optimizing the IDS model by extracting rules using GA. To add transparency in the decision-making process, Dias et al., in \cite{dias2021hybrid} proposed an interpretable and explainable hybrid intrusion detection system. The proposed system integrates expert-written rules and dynamic knowledge generated by a DT algorithm. The authors suggest that the model can achieve explainability and interpretability through the justifications of each diagnosis. The justification for a certain prediction is provided in the form of a suggested rule. 

    
     \subsubsection{Statistical and Probabilistic Methods}
     \label{Statistical and Probabilistic Models}
     %In most cases, statistical approaches begin by constructing a statistical model based on the available data, and then use a statistical inference test to evaluate if an unknown occurrence fits into that model or not. It then flags instances that have a low likelihood of occurrence from the learned model as probable intrusions/anomalies. In essence, statistical Anomaly Intrusion Detection System (AIDS) considers the median, mean, mode, and standard deviation of packets among other statistical metrics. Rather than inspecting data traffic, each packet is monitored, capturing the flow's fingerprint. This approach is used to discover any deviation from normal behavior.
     
     %Published surveys on AIDS have categorized statistical approaches into three models including univariate model, multivariate model, time series model \cite{khraisat2019survey}.  Some recent surveys have broken down the statistical approach for network anomaly detection into two categories namely, parametric, and non-parametric \cite{bhuyan2013network}, \cite{tran2017network}. Papers ranging from 2005 - 2012 categorized statistical analysis techniques into five categories namely, Operational model, Markov model, Statistical moments, Multivariate, and Times Series \cite{qayyum2005taxonomy}, \cite{gyanchandani2012taxonomy}. 
     
     %Mean and standard deviations: In statistics, the mean, standard deviation, and any other type of correlation are referred to as moments \cite{qayyum2005taxonomy}, \cite{jyothsna2011review}. When events occur either above or below a predefined interval, a moment is said to be anomalous \cite{hodo2017shallow}. The authors in \cite{ashfaq2010information} proposed a novel information-theoretic combining method that takes into account the accuracy of the individual classifiers in a multi-classifier Network Anomaly Detection System. (NADS). A Standard Deviation normalized Entropy of Accuracy (SDnEA) method is used for classifier combining. Two real traffic dataset was used in this work such as Lawrence Berkeley National Laboratory (LBNL) and the Endpoint dataset. The proposed model showed promising performance in detection rate with 3\% - 10\% increment and 40\% decrement in false alarm rate. 
     
    % Multivariate Models : Multivariate models are analogous to the mean-standard deviation model \cite{qayyum2005taxonomy}, \cite{kuperman2004categorization}. The major difference is these models are based on correlations among two or more metrics. W.Sha et al. \cite{sha2013multi} took into account multivariate time series and high-order Markov chains in addition to the detailed design of training and testing algorithms for anomaly detection in server systems. To evaluate the effectiveness of the model, the researchers used the DARPA dataset. Experimental results indicated this approach can produce several effective indicators of anomalies. 
     
     %Markov Process: Markov processes can be approached in two ways: through Markov chains or hidden Markov models. \cite{ye2000markov} demonstrated an anomaly detection technique based on the Markov chain model. A Markov chain is used in this method to represent the temporal profile of normal behavior in a computer or network system. The normal profile Markov chain model is learned from historical data and the system's observed behavior is compared to the Markov chain model of normal behavior. A low resemblance between these two behaviors indicates the presence of intrusions. 

    In statistics, the mean, standard deviation, and any other type of correlation are referred  to as moments \cite{qayyum2005taxonomy}, \cite{jyothsna2011review}. 
    Statistical and probabilistic methods use this information to determine whether the given event is anomalous or not. The moment is predicted anomalous if they are either above or below a predefined interval \cite{hodo2017shallow}.
 This approach is further divided into the univariate model, multivariate model, time series model in \cite{khraisat2019survey}, parametric and non-parametric model in \cite{bhuyan2013network}, \cite{tran2017network}, operational model, Markov model and statistical moments in \cite{qayyum2005taxonomy}, \cite{gyanchandani2012taxonomy}.

    %In statistics, the mean, standard deviation, and any other type of correlation are referred to as moments \cite{qayyum2005taxonomy}, \cite{jyothsna2011review}. When events occur either above or below a predefined interval, a moment is said to be anomalous \cite{hodo2017shallow}. 
    Various IDS based on statistical and probabilistic models have been proposed. IDS based on the mean and standard deviation is explained in \cite{ashfaq2010information}, while a study relating to multivariate modeling is proposed in \cite{sha2013multi}. The authors in \cite{ye2000markov} proposed an IDS based on the Markov process. 
    

    A different approach to intrinsically explainable statistical methods for network intrusion detection is proposed by Pontes et al. \cite{pontes2021new}. The authors in this study introduce a novel Energy-based Flow Classifier (EFC) that utilizes inverse Potts models to infer anomaly scores based on labeled benign examples. This method is capable of accurately performing binary flow classification on DDoS attacks. They perform experiments on three different datasets: CIDDS-001, CIC-IDS2017, and CICDDoS19. Results indicate that the proposed model is more adaptable to different data distributions than classical ML-based classifiers. Additionally, they argue that their model is naturally interpretable and that individual parameter values can be analyzed in detail.  
    
    %They perform experiments on three different datasets: CIDDS-001, CIC-IDS2017, and CICDDoS19, which shows that it is more adaptable to different data distributions than classical ML-based classifiers. They further argue that the proposed model is naturally interpretable and can be analyzed in detail regarding individual parameter values. The white box nature of the proposed statistical model \hl{inferred by EFC} is demonstrated by breaking down different attack classes into individual contributions of each pair of features.

     
     
\subsubsection{Clustering}
Clustering is the most widely used strategy for unsupervised ML. It classifies samples according to a similarity criterion. %, such that samples belonging to the same group are comparable to those belonging to another. 
Clustering algorithms that can be explained have several advantages. The primary benefit of explainable clustering is that it summarizes the input behavior patterns within clusters, enabling users to comprehend the clusters' underlying commonalities \cite{wickramasinghe2021explainable}. As stated in Section \ref{overview_whitebox_approach} there are various clustering algorithms available. However, in the context of X-IDS, we will only focus on Self-Organizing Maps (SOMs).

SOMs are an unsupervised clustering technique within the artificial neural networks umbrella. It has two layers: an input layer that accepts high dimensional space and an output layer that generates a non-linear mapping of high-dimensional space into reduced dimensions.  It is trained to produce a low dimensional representation of a large training dataset while preserving important topological and metric relationships of the input data \cite{kohonen1996engineering}. A graphical illustration of a simple SOM model is depicted in Figure \ref{fig: SOM}.
    \begin{figure}[h!]
    \centerline{\includegraphics[scale =0.55 ]{figures/SOM.pdf}}
    \caption{Clustering based on Self Organizing Maps. The input layer consists of $x_{0}, x_{1}...x_{n}$ nodes. These nodes have specific weights illustrated by $w_{00}, w_{01},...w_{n1}$. These weight determines cluster classification such as $C_{0}$ and $C_{1}$.}
    \label{fig: SOM}
    \end{figure}

%\indent The authors in \cite{wickramasinghe2021explainable} developed a novel model-specific explainable technique for the SOM algorithm that generates both local and global explanations for Cyber-Physical Systems. They used the SOMs training approach (winner-take-all algorithm) together with visual data mining capabilities (Histograms, t-SNE, Heat Maps, and U-Matrix) of SOM to make the algorithm explainable. In this work, the authors used four different algorithms. The first algorithm is used to train SOM with dimension \textit{d*d}. The order of important features is then calculated on the trained dataset using algorithm 2. The authors use standard deviation to decide the importance of a feature. They then calculate the ordered list of important features of each neuron. The feature indices are sorted from lowest to highest standard deviation, corresponding to an ordered list of features ranked from highest to lowest in terms of importance. For interpretability purposes, the authors clustered SOM neurons using K-Means clustering. Furthermore, two experiments were designed to determine the importance of the identified features for each neuron in the SOM decision-making process also referred to as a fidelity test on the test dataset. The first experiment was used to calculate the percentage of change in cluster labels when changing the feature value of an important feature using algorithm three. The second experiment, using algorithm four, was to check if the calculated order of the important feature lists was correct for the test dataset. Five datasets were used in the experiment including KDD, German Credit, Bank marketing, Adult Income, and DoHBrw-2020. 70\% of the data was chosen at random for training, with the remainder used for testing. Experimental results indicated that the proposed method identifies the most important features responsible for the decision-making process of SOM.

%A host-based automatic anomaly detection system was proposed by Hoglund et al. \cite{hoglund2000computer}. At first, the system builds a normal model by collecting the normal data from UNIX audit data (user behavior). This model is subsequently used to detect if the current behavior of an object is anomalous or not using the SOM technique. The authors conducted a hypothesis-based experiment; the null hypothesis \textit{H$_{0}$} – the most recent observation is not anomalous and the alternative hypothesis \textit{H$_{1}$} – the most recent observation is anomalous. SOMs are trained using the procedures of SOM\_PAK. One of the major shortcomings of the proposed system is that this system does not cater the real-time detection, it only works with past user log data. The proposed system still needs human expert knowledge during the feature selection process, which is a manual process. \\
  %\indent On the other hand, unlike the systems based on audit trails as proposed by Hoglund et al. \cite{hoglund2000computer}, the authors in \cite{lichodzijewski2002host} proposed Hierarchical SOMs for host-based intrusion detection on computer networks that are capable of operating on real-time data without requiring extensive offline training or expert knowledge. In this work, UNIX ``session information" is used to define the system's features, as well as the characteristics of a common user. To discover the pattern and to visualize the characteristics of a common user, the authors use two-tiered hierarchical SOM architecture. The first level is made up of three maps. The first map is based on location data, the second is based on the user account from which the login connection is made, and the third map is connection type. The second level, on the other hand, receives the output of the first level as its input and combines the results into a unified summary of user activity. This output from the second level indicates whether a particular session is abnormal or not. The data for this experiment was extracted from the UNIX log files of the authors institution’s undergraduate host machine. This host has nearly 2300 user accounts and is primarily used for email and coursework by undergraduate students. To detect intrusions, different SOMs are fed different types of data, which is then summarized by a SOM. Along with reducing training data size, the hierarchical structure reduces computational overhead. \\
   %\indent Kayacik HG et al. \cite{kayacik2007hierarchical} proposed an approach to detect network intrusion based on hierarchical SOM architecture. The proposed method is evaluated using two different basic feature sets: one that contains only six basic features and another that contains all 41 features from the KDD99 dataset. The experiment demonstrates that the optimal performance can be achieved by combining all 41 features with two SOM layers, or by combining six features with three layers. The authors asserted that only 40\% of data was sufficient for training purposes. Experimental results indicated the proposed system produced 1.38\% false positives and achieved 90.4\% detection rates under the test conditions. According to the authors, intrusion detection should be built around protocol and service features. They suggested that the of the 6 features including protocol type, status flag, connection, total bytes sent to the destination host, total bytes sent to the source host, and service type, the only feature that increases false-positive and detection rates is the protocol type. Eliminating any of the remaining five features resulted in lower false-positive and detection rates for detection systems.   

An anomaly detection system using SOM techniques based on offline audit trail data is proposed in \cite{hoglund2000computer}. The major shortcoming of the proposed system is it does not allow for real-time detection. On the other hand, the authors in \cite{lichodzijewski2002host} propose Hierarchical SOMs (HSOM) for host-based intrusion detection on computer networks that are capable of operating on real-time data without requiring extensive offline training or expert knowledge. Another model based on HSOM is proposed in \cite{kayacik2007hierarchical}. %This study aims to reduce false-positive and increase detection accuracy. 
The authors in \cite{wickramasinghe2021explainable} developed a novel model-specific explainable technique for the SOM algorithm that generates both local and global explanations for Cyber-Physical Systems (CPS) security. They used the SOMs training approach (winner-take-all algorithm) together with visual data mining capabilities (Histograms, t-SNE, Heat Maps, and U-Matrix) of SOMs to make the algorithm explainable. %In this work, the authors used four different algorithms. The first algorithm is used to train SOM with dimension \textit{d*d}. The order of important features is then calculated on the trained dataset using algorithm 2. The authors use standard deviation to decide the importance of a feature. They then calculate the ordered list of important features of each neuron. The feature indices are sorted from lowest to highest standard deviation, corresponding to an ordered list of features ranked from highest to lowest in terms of importance. For interpretability purposes, the authors clustered SOM neurons using K-Means clustering. Furthermore, two experiments were designed to determine the importance of the identified features for each neuron in the SOM decision-making process also referred to as a fidelity test on the test dataset. The first experiment was used to calculate the percentage of change in cluster labels when changing the feature value of an important feature using algorithm three. The second experiment, using algorithm four, was to check if the calculated order of the important feature lists was correct for the test dataset. Five datasets were used in the experiment including KDD, German Credit, Bank marketing, Adult Income, and DoHBrw-2020. 70\% of the data was chosen at random for training, with the remainder used for testing. Experimental results indicated that the proposed method identifies the most important features responsible for the decision-making process of SOM.
   
A 3D color hexagonal SOM for visual intrusion detection called ANNaBell Island is proposed in \cite{langin2011annabell} which is an extension of 1D ANNaBell reported in \cite{ langin2008model, langin2009self}. To make the SOM process and its output explainable to the users, the authors designed a hexagonal SOM in a meta-hexagonal layout, referred to as an island, that graphically displayed features of network traffic. The output of the SOM model was used to create a color-separated 3D landscaped island that represents various types of network traffic, distinguishing between malicious and normal behavior.

After surveying the current black box and white box approaches to X-IDS, we propose in the next section, a generic explainable architecture with a user-centric approach for designing X-IDS that can accommodate a wide variety of scenarios and applications without adhering to a specification or technological solution.


